Fast reconstruction of atomic-scale STEM-EELS images from sparse sampling

This paper discusses the reconstruction of partially sampled spectrum-images to accelerate the acquisition in scanning transmission electron microscopy (STEM). The problem of image reconstruction has been widely considered in the literature for many imaging modalities, but only a few attempts handled 3D data such as spectral images acquired by STEM electron energy loss spectroscopy (EELS). Besides, among the methods proposed in the microscopy literature, some are fast but inaccurate while others provide accurate reconstruction but at the price of a high computation burden. Thus none of the proposed reconstruction methods fulfills our expectations in terms of accuracy and computation complexity. In this paper, we propose a fast and accurate reconstruction method suited for atomic-scale EELS. This method is compared to popular solutions such as beta process factor analysis (BPFA) which is used for the first time on STEM-EELS images. Experiments based on real as synthetic data will be conducted.

==> sections/hidden.tex <==
\begin{table}[htbp]
    \centering
    \bgroup
        \renewcommand{\arraystretch}{1.2}
        
        \subfigure[HR1]{
            \begin{tabular}{%
                    c%
                    c%
                    c%
                    c}%
                \toprule
                Method& 
                SNR&
                aSAD (100$\times$)&
                Exec. time\\
                %
                \midrule
                %
                NN     & 30.81 & 1.384 & \textbf{0.26s}\\
                3S     & 32.32 & 1.066 & 6.21s\\
                \FS{}  & 36.18 & \textbf{1.061} & 7.72s\\
                ITKrMM & 36.75 & 1.087 & 1h35m55.41s\\
                wKSVD  & 36.97 & 1.091 & 12h18m43.32s\\
                BPFA   & \textbf{37.02} & 1.089 & 37h36m17.43s\\
                \bottomrule
            \end{tabular}
        }
        %
        \subfigure[HR2]{
            \begin{tabular}{%
                    c%
                    c%
                    c%
                    c}%
                \toprule
                Method& 
                SNR&
                aSAD (100$\times$)&
                Exec. time\\
                %
                \midrule
                %
                NN     & 28.70 & 1.821 & \textbf{0.06s}\\
                3S     & 30.16 & 1.499 & 1.26s\\
                \FS{}  & 33.18 & 1.240 & 0.41s\\
                ITKrMM & 33.92 & 1.211 & 16m1.70s\\
                wKSVD  & 34.53 & 1.168 & 1h46m16.92s\\
                BPFA   & \textbf{34.98} & \textbf{1.108} & 5h29m33.25s\\
                %
                \bottomrule
            \end{tabular}
        }
        %
        \subfigure[Synth]{
            \begin{tabular}{%
                    c%
                    c%
                    c%
                    c}%
                \toprule
                Method& 
                SNR&
                aSAD (100$\times$)&
                Exec. time\\
                %
                \midrule
                %
                NN     & 21.32 & 1.462 & \textbf{0.03s}\\
                3S     & 22.12 & 1.188 & 1.60s\\
                \FS{}  & 42.16 & 0.224 & 1.28s\\
                ITKrMM & 45.89 & 0.247 & 13m26.98s\\
                wKSVD  & 45.78 & 0.271 & 1h38m35.81s\\
                BPFA   & \textbf{52.94} & \textbf{0.149} & 3h19m5.68s\\
                %
                \bottomrule
            \end{tabular}
        }
    \egroup
    \caption{The SNR and aSAD metric values for all data and methods. The execution time is also given to be considered jointly with accuracy.}
    \label{table:results-time}
\end{table}






\begin{figure*}
    \centering
    
    \begin{tikzpicture}[]
        \pgfplotsset{every axis plot/.append style={line width=1pt,}}
        \begin{groupplot}[
            group style={
                group size=3 by 1,
                group name=plots,
            },
            %
            ymode=log,
            %
            xlabel={$r$},
            label style={font=\small},
            %
            width=0.33\textwidth,
            height=0.7\columnwidth,
            ]
            %
            \nextgroupplot[% 1
                ylabel={Reconstruction error},
                ]
                \addplot+ [] table [x=rTab, y=fourier]{img/2.basis/HR1.dat};
                \addplot+ [] table [x=rTab, y=dct]{img/2.basis/HR1.dat};
                \addplot+ [] table [x=rTab, y=db3]{img/2.basis/HR1.dat};
                \addplot+ [] table [x=rTab, y=db10]{img/2.basis/HR1.dat};
                \addplot+ [] table [x=rTab, y=db20]{img/2.basis/HR1.dat};
                \addplot+ [] table [x=rTab, y=sym3]{img/2.basis/HR1.dat};
                \addplot+ [] table [x=rTab, y=sym10]{img/2.basis/HR1.dat};
                \addplot+ [] table [x=rTab, y=sym20]{img/2.basis/HR1.dat};
            %
            \nextgroupplot[% 2
                legend entries={Fourier, DCT, db3, db10, db20, sym3, sym10, sym20},
                legend style={
                    draw=none, 
                    at={(0.5,1.03)}, 
                    anchor=south, 
                    legend columns=8, 
                    /tikz/every even column/.append style={column sep=0.5cm}
                },
                ]
                \addplot+ [] table [x=rTab, y=fourier]{img/2.basis/HR2.dat};
                \addplot+ [] table [x=rTab, y=dct]{img/2.basis/HR2.dat};
                \addplot+ [] table [x=rTab, y=db3]{img/2.basis/HR2.dat};
                \addplot+ [] table [x=rTab, y=db10]{img/2.basis/HR2.dat};
                \addplot+ [] table [x=rTab, y=db20]{img/2.basis/HR2.dat};
                \addplot+ [] table [x=rTab, y=sym3]{img/2.basis/HR2.dat};
                \addplot+ [] table [x=rTab, y=sym10]{img/2.basis/HR2.dat};
                \addplot+ [] table [x=rTab, y=sym20]{img/2.basis/HR2.dat};
            %
            \nextgroupplot% 3
                \addplot+ [] table [x=rTab, y=fourier]{img/2.basis/Synth.dat};
                \addplot+ [] table [x=rTab, y=dct]{img/2.basis/Synth.dat};
                \addplot+ [] table [x=rTab, y=db3]{img/2.basis/Synth.dat};
                \addplot+ [] table [x=rTab, y=db10]{img/2.basis/Synth.dat};
                \addplot+ [] table [x=rTab, y=db20]{img/2.basis/Synth.dat};
                \addplot+ [] table [x=rTab, y=sym3]{img/2.basis/Synth.dat};
                \addplot+ [] table [x=rTab, y=sym10]{img/2.basis/Synth.dat};
                \addplot+ [] table [x=rTab, y=sym20]{img/2.basis/Synth.dat};
            %
        \end{groupplot}

        \draw ($(plots c1r1.south) - (0, 1.5)$) node {\small(a) HR1};
        \draw ($(plots c2r1.south) - (0, 1.5)$) node {\small(b) HR2};
        \draw ($(plots c3r1.south) - (0, 1.5)$) node {\small(c) Synth};

    \end{tikzpicture}
    %
    \caption{Reconstruction error for several bases. The faster the curve decreases, the better as it means the image needs less representation coefficients to accurately represented. The DCT basis gives the best results for all images.}
    \label{fig:best-basis}
\end{figure*}




\renewcommand{\myplot}[1]{
    \begin{axis}[
        %
        xlabel={Energy loss (eV)},
        ylabel={Amplitude},
        %
        legend entries={Reference, NN, 3S, \FS{}, ITKrMM, wKSVD, BPFA},%
        %
        width=\textwidth,
        height=0.3\textwidth,
        %
        % legend
        legend style={
            draw=none, 
            at={(0.5,1.03)}, 
            anchor=south, 
            legend columns=8, 
            /tikz/every even column/.append style={column sep=0.5cm}
        },
        axis background/.style={fill=white},
        line width=#1,
        ]
        \addplot+ [] table [x=eV, y=GT]{\fileplot};
        \addplot+ [] table [x=eV, y=NN]{\fileplot};
        \addplot+ [] table [x=eV, y=SSS]{\fileplot};
        \addplot+ [] table [x=eV, y=FS3D]{\fileplot};
        \addplot+ [] table [x=eV, y=ITKrMM]{\fileplot};
        \addplot+ [] table [x=eV, y=wKSVD]{\fileplot};
        \addplot+ [] table [x=eV, y=BPFA]{\fileplot}; 
    \end{axis}
}

\renewcommand{\myplott}[1]{
    \begin{axis}[
        %
        xlabel={Energy loss (eV)},
        ylabel={Amplitude},
        %
        legend entries={Reference, NN, 3S, \FS{}, ITKrMM, wKSVD, BPFA},%
        %
        width=\textwidth,
        height=0.3\textwidth,
        %
        xmin=815,
        xmax=840,
        % legend
        legend style={
            draw=none, 
            at={(0.5,1.03)}, 
            anchor=south, 
            legend columns=8, 
            /tikz/every even column/.append style={column sep=0.5cm}
        },
        axis background/.style={fill=white},
        line width=#1,
        ]
        \addplot+ [] table [x=eV, y=GT]{\fileplot};
        \addplot+ [] table [x=eV, y=NN]{\fileplot};
        \addplot+ [] table [x=eV, y=SSS]{\fileplot};
        \addplot+ [] table [x=eV, y=FS3D]{\fileplot};
        \addplot+ [] table [x=eV, y=ITKrMM]{\fileplot};
        \addplot+ [] table [x=eV, y=wKSVD]{\fileplot};
        \addplot+ [] table [x=eV, y=BPFA]{\fileplot}; 
    \end{axis}
}



\subfigure[Sampled pixel (blue pixel)]{
    %
    \def\filetmp{\fileplot}
    %
    \begin{tikzpicture}[]
        \myplot{1pt}
    
        \fill [opacity=0.2, blue] (10.4, 0.3) rectangle (10.9, 4);
    
        \draw [blue, line width=1pt,  drop shadow](14, 0.1) rectangle (16.25, 3.8);

    \begin{scope}[xshift=14cm, yshift=-0.2cm]
        \begin{scope}[xscale=4.5, xshift=-10.4cm]
            
            \clip[draw] (10.4, 0.3) rectangle (10.9, 4);
            \myplot{0.1pt}
        
        \end{scope}
    \end{scope}
    
\draw [blue, line width=1pt] (14, 0.1) rectangle (16.25, 3.8);
          
\end{tikzpicture}
        %
        \label{subfig:synth_spectra_samp}
}\\
    %    
    \subfigure[Non-sampled pixel (red pixel)]{
        %
        \def\fileplot{img/3.synth_im/synth_HR2_non_samp.dat}
        \input{img/spectra_template_no_legend}
        %
        \label{subfig:synth_spectra_non_samp}
    }




\begin{tikzpicture}[]
    
    \myplott{0.5pt}
    
\end{tikzpicture}

\begin{comment}
\begin{tikzpicture}[]
    
    \myplot{1pt}
    
    \fill [opacity=0.2, blue] (10.4, 0.3) rectangle (10.9, 4);
    
    \draw [blue, line width=1pt,  drop shadow](14, 0.1) rectangle (16.25, 3.8);

    \begin{scope}[xshift=14cm, yshift=-0.2cm]
        \begin{scope}[xscale=4.5, xshift=-10.4cm]
            
            \clip[draw] (10.4, 0.3) rectangle (10.9, 4);
            \myplot{0.1pt}
        
        \end{scope}
    \end{scope}
    
\draw [blue, line width=1pt] (14, 0.1) rectangle (16.25, 3.8);
          
\end{tikzpicture}
\end{comment}


\renewcommand{\myplot}[1]{
    \begin{axis}[
        %
        xlabel={Energy loss (eV)},
        ylabel={Amplitude},
        %
        width=\textwidth,
        height=0.3\textwidth,
        %
        % legend
        legend style={
            draw=none, 
            at={(0.5,1.03)}, 
            anchor=south, 
            legend columns=8, 
            /tikz/every even column/.append style={column sep=0.5cm}
        },
        axis background/.style={fill=white},
        line width=#1,
        ]
        \addplot+ [] table [x=eV, y=GT]{\fileplot};
        \addplot+ [] table [x=eV, y=NN]{\fileplot};
        \addplot+ [] table [x=eV, y=SSS]{\fileplot};
        \addplot+ [] table [x=eV, y=FS3D]{\fileplot};
        \addplot+ [] table [x=eV, y=ITKrMM]{\fileplot};
        \addplot+ [] table [x=eV, y=wKSVD]{\fileplot};
        \addplot+ [] table [x=eV, y=BPFA]{\fileplot}; 
    \end{axis}
}

\begin{tikzpicture}[]
    
    \myplot{1pt}
    
    \fill [opacity=0.2, blue] (10.4, 0.3) rectangle (10.9, 4);
    
    \draw [blue, line width=1pt,  drop shadow](14, 0.1) rectangle (16.25, 3.8);

    \begin{scope}[xshift=14cm, yshift=-0.2cm]
        \begin{scope}[xscale=4.5, xshift=-10.4cm]
            
            \clip[draw] (10.4, 0.3) rectangle (10.9, 4);
            \myplot{0.1pt}
        
        \end{scope}
    \end{scope}
    
\draw [blue, line width=1pt] (14, 0.1) rectangle (16.25, 3.8);
          
\end{tikzpicture}


==> table/synth_error_im_results.tex <==
\begin{tabular}{m{1.5cm}*{3}{>{\centering\arraybackslash}m{1.02\mycolwidth}}}
    Sampling mask&
    \includegraphics[width=\mycolwidth]{img/4.real_im/real_im/mask.png}&
    &
    \\
    %
    Component&
    {$\mathrm{O-K}$}&
    {$\mathrm{La-M}_{4, 5}$}&
    {$\mathrm{Nd-M}_{4, 5}$}\\
    %
    Reference&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/error_HR2/HR2_GT_band_0.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/error_HR2/HR2_GT_band_1.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/error_HR2/HR2_GT_band_2.png}\\
    NN&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/error_HR2/HR2_interpolation_band_0.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/error_HR2/HR2_interpolation_band_1.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/error_HR2/HR2_interpolation_band_2.png}\\
    3S&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/error_HR2/HR2_3S_band_0.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/error_HR2/HR2_3S_band_1.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/error_HR2/HR2_3S_band_2.png}\\
    \CLS{}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/error_HR2/HR2_CLS_band_0.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/error_HR2/HR2_CLS_band_1.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/error_HR2/HR2_CLS_band_2.png}\\
    ITKrMM&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/error_HR2/HR2_ITKrMM_matlab_band_0.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/error_HR2/HR2_ITKrMM_matlab_band_1.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/error_HR2/HR2_ITKrMM_matlab_band_2.png}\\
    wKSVD&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/error_HR2/HR2_wKSVD_matlab_band_0.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/error_HR2/HR2_wKSVD_matlab_band_1.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/error_HR2/HR2_wKSVD_matlab_band_2.png}\\
    BPFA&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/error_HR2/HR2_BPFA_matlab_band_0.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/error_HR2/HR2_BPFA_matlab_band_1.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/error_HR2/HR2_BPFA_matlab_band_2.png}\\
\end{tabular}

==> table/synth_im_results.tex <==
\begin{tabular}{m{1.5cm}*{3}{>{\centering\arraybackslash}m{1.02\mycolwidth}}}
    Sampling mask&
    \includegraphics[width=\mycolwidth]{img/4.real_im/real_im/mask.png}&
    &
    \\
    %
    Component&
    {$\mathrm{O-K}$}&
    {$\mathrm{La-M}_{4, 5}$}&
    {$\mathrm{Nd-M}_{4, 5}$}\\
    %
    Reference&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/HR2/0/HR2_0_GT_band_0.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/HR2/0/HR2_0_GT_band_1.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/HR2/0/HR2_0_GT_band_2.png}\\
    NN&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/HR2/0/HR2_0_NN_band_0.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/HR2/0/HR2_0_NN_band_1.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/HR2/0/HR2_0_NN_band_2.png}\\
    3S&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/HR2/0/HR2_0_SSS_band_0.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/HR2/0/HR2_0_SSS_band_1.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/HR2/0/HR2_0_SSS_band_2.png}\\
    \CLS{}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/HR2/0/HR2_0_FS3D_band_0.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/HR2/0/HR2_0_FS3D_band_1.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/HR2/0/HR2_0_FS3D_band_2.png}\\
    ITKrMM&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/HR2/0/HR2_0_ITKrMM_band_0.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/HR2/0/HR2_0_ITKrMM_band_1.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/HR2/0/HR2_0_ITKrMM_band_2.png}\\
    wKSVD&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/HR2/0/HR2_0_wKSVD_band_0.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/HR2/0/HR2_0_wKSVD_band_1.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/HR2/0/HR2_0_wKSVD_band_2.png}\\
    BPFA&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/HR2/0/HR2_0_BPFA_band_0.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/HR2/0/HR2_0_BPFA_band_1.png}&
    \includegraphics[width=\mycolwidth]{img/3.synth_im/HR2/0/HR2_0_BPFA_band_2_size.png}\\
\end{tabular}
